Certifying Safety in Reinforcement Learning under Adversarial Perturbation Attacks

Function approximation has enabled remarkable advances in applying reinforcement learning (RL) techniques in environments with high-dimensional inputs, such as images, in an end-to-end fashion, mapping such inputs directly to low-level control. Nevertheless, these have proved vulnerable to small adversarial input perturbations. A number of approaches for improving or certifying robustness of end-to-end RL to adversarial perturbations have emerged as a result, focusing on cumulative reward. However, what is often at stake in adversarial scenarios is the violation of fundamental properties, such as safety, rather than the overall reward that combines safety with efficiency. Moreover, properties such as safety can only be defined with respect to true state, rather than the high-dimensional raw inputs to end-to-end policies. To disentangle nominal efficiency and adversarial safety, we situate RL in deterministic partially-observable Markov decision processes (POMDPs) with the goal of maximizing cumulative reward subject to safety constraints. We then propose a partially-supervised reinforcement learning (PSRL) framework that takes advantage of an additional assumption that the true state of the POMDP is known at training time. We present the first approach for certifying safety of PSRL policies under adversarial input perturbations, and two adversarial training approaches that make direct use of PSRL. Our experiments demonstrate both the efficacy of the proposed approach for certifying safety in adversarial environments, and the value of the PSRL framework coupled with adversarial training in improving certified safety while preserving high nominal reward and high-quality predictions of true state.

==> certify.tex <==
\section{Certification}
We present algorithms for certification under both $l_2$ and $l_\infty$ norms. For both norms, the certification process for the reinforcement learning part are the same, which is to use $\alpha/\beta$-crown \cite{xu2021fast,wang2021betacrown} to calculate the upper/lower bound of Q values; based on the bounds of Q values, we calculate the actions that could possibly be taken: any action that the upper bound of the Q value is higher than the maximum lower bound among all actions. The only difference between $l_2$ and $l_\infty$ norms is how the bounds for the features are derived, which we name it as the CV component, note that the CV component is the input to the RL component.

\subsection{RL Certification}
For the certification of the RL, we grow the action tree by slowly increase the target adversarial attack budget $\epsilon$. We create the following data structure for each node of the tree; where each node corresponds to a state. 

A node of the tree has the below elements
\begin{itemize}
    \item state of the node: this could be the sequence of actions that has been taken to reach the state of the node; or the state representation which we could recover the simulator to (e.g., a deepcopy of the gym environment).
    \item children lists: a list that store the child nodes of the current node.
    \item step level: the depth of the current node in the tree; this is to stop growing the tree when the desired number of steps we hope to verify is reached.
    \item action taken: the next possible actions set given the state of the current node and the current $\epsilon$ we are certifying against; in other words, the actions set it takes to reach all possible children nodes.
    \item robust epsilon: the maximum epsilon the current node is robust against for the ``action taken" set. By definition, this should be no smaller than the current $\epsilon$ we are certifying against.
    \item action next: if the epsilon is greater than current $\epsilon_i$ (i.e., if it is $\epsilon_{i+1}$), what are the additional actions to be possibly taken (or in other words, to be included into action taken).
    \item max safety epsilon: the minimum of ``max safety epsilon" of all the children nodes, as well as the ``robust epsilon" of the current node. For nodes without childnode, the value is 255.0 (or any sufficiently large number).
\end{itemize}

For every step iteration, we set the ``target epsilon" equal to the max safety epsilon (global, i.e., max safety epsilon of the root node), and further expand the nodes whose ``robust epsilon" is equal to the target epsilon by adding children whose action correspond to the actions in ``action next"; furthermore, if the ``max safety epsilon" of the tree node is greater than  the ``target epsilon", we skip the node as well as its child nodes. Note that here by definition, the max safety epsilon of all nodes is no less than the global max safety epsilon.

\subsection{CV Certification}
For $l_\infty$ norm, we use $\alpha/\beta$-crown to calculate the upper and lower bound of each features; for $l_2$ norm, we use median-smoothing \cite{chiang2020detection} to calculate the upper/lower bound of each features.
\begin{lemma}
\label{pert_smooth}
A percentile-smoothed function $h_p$ with adversarial perturbation $\delta$ can be bounded as
\begin{equation}
    h_{\underline{p}}(x) \leq h_{p}(x+\delta) \leq h_{\bar{p}}(x) \quad \forall\|\delta\|_{2}<\epsilon,
\end{equation}
where $h_p(x) = \{y\in\mathbb{R}|\mathbb{P}[f(x+G)\leq y ] = p\}, G\sim N(0,\sigma^2I)$ (the $p$-th percentile), $\underline{p}:=\Phi\left(\Phi^{-1}(p)-\frac{\epsilon}{\sigma}\right)$ and $\bar{p}:=\Phi\left(\Phi^{-1}(p)+\frac{\epsilon}{\sigma}\right)$, with $\Phi$ being the standard Gaussian CDF.
\end{lemma}
The full algorithm is as below
\begin{algorithm}[htbp]
\caption{Safety verification}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithmic}[1]
\REQUIRE NN for the RL agent, NN for the CV part, EpisodeLength
\ENSURE $\epsilon_\text{safety}$ ($\epsilon$ where safety is guaranteed)
\STATE Grow the tree without any adversarial perturbation (i.e., all actions are clean action).
\IF{ego vehicle is unsafe w.r.t. other vehicles}
\STATE $\epsilon_\text{safety}\leftarrow 0$
\RETURN $\epsilon_\text{safety}$
\ENDIF
\STATE Update ``max safety epsilon" of the tree.
\WHILE{TRUE}
\STATE $\epsilon_\text{next} \leftarrow$ ``max safety epsilon" of the RootNode
\STATE \textsc{TreeExpand}(RootNode, $\epsilon_\text{next}$)
\STATE Update ``max safety epsilon" of the tree.
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htbp]
\caption{\textsc{TreeExpand}(CurrentNode, $\epsilon$)}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithmic}[1]
\IF{CurrentNode.MaxSafetyEpsilon  $>\epsilon$}
\STATE Pass
\ELSE
\FOR{ChildNode in CurrentNode.ChildNodeList}
\STATE \textsc{TreeExpand}(ChildNode, $\epsilon$)
\IF{ChildNode.StepLevel == EpisodeLength}
\STATE Pass
\ELSIF{ChildNode.RobustEpsilon == $\epsilon$}
\STATE \textsc{GrowTree}(ChildNode, $\epsilon$)
\ENDIF
\ENDFOR
\ENDIF
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htbp]
\caption{\textsc{GrowTree}(CurrentNode, $\epsilon$)}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithmic}[1]
\STATE ExpandQueue $\leftarrow$ [ ]
\STATE Initialize nodes that corresponds to actions in CurrentNode.ActionNext, push those nodes to ExpandQueue
\STATE Update the information of CurrentNode (e.g., ChildList, ActionNext, ActionTaken, RobustEpsilon)
\WHILE{ExpandQueue is not empty}
\STATE Pop ExpandNode from ExpandQueue (follow FILO rule)
\STATE Grow ExpandNode one depth further, with RobustEpsilon for each node $\geq \epsilon + 1.0/255$.
\IF{ego vehicle is unsafe w.r.t. other vehicles}
\RETURN $\epsilon_\text{safety} = \epsilon$
\ENDIF
\IF{Depth(ExpandNode.Children) $<$ EpisodeLength}
\STATE Push ExpandNode.Children to ExpandQueue
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> generalizations.tex <==
\section{Generalizations}
\label{S:general}

Our system model is a POMDP with a deterministic transition $\tau$ and observation $f$ functions.
We now show how our approach can be applied even when neither of these assumptions hold.
The simpler case is deterministic transitions $o=f(s)$: in fact, nothing in the proposed PSRL, certification, or adversarial training needs this assumption.
Rather, it suffices for our purposes that every observation $o \in O$ corresponds to a unique state $s$, but observations can indeed be stochastic given a state $s$. 
Our assumption of deterministic transition $\tau$ can also be relaxed.
Specifically, it suffices for our purposes to assume that for each state $s$ and action $a$, the probability distribution $\tau(s,a) = \Pr\{s'|s,a\}$ has a finite support $D(s,a)$.
Then, whenever we expand an action $a$ at a node corresponding to state $s$ during verification, we expand the entire set $D(s,a)$, and reason over the induced subtree for each $s' \in D(s,a)$.

==> training.tex <==
\section{OLD: Learning Robust Policies}
\subsection{$l_\infty$ norm}
We experiment on 3 types of loss functions:
\begin{enumerate}
    \item Treat 2 NN (CV and RL) as one, where for the RL part we use the RADIAL loss function, and for CV part we only train to minimize the MSE with the predicted feature and true feature.
    \item Treat 2 NN separately, where for the CV part we minimize the MSE of the predicted (clean) feature and true feature, plus the MSE of the predicted (adversarial perturbed) feature and true feature -- more precisely, minimize the MSE of lower and upper bound to the true feature. Similarly to the RADIAL loss function for the RL part, we assign weight $(1-\kappa)$ to the MSE of the predicted (clean) feature and true feature, and $\kappa$ to the MSE of the predicted (adversarial perturbed) feature and true feature. For the RL part, we use the upper/lower bound of the features as the input bounds to IBP (we treat them as constant values), and then apply RADIAL loss function to it.
    \item This method is a hybrid combination of the previous two methods, where we have the RL loss function, where we treat 2NN as one; and we also have the CV loss function, which minimize the MSE of the predicted (clean) feature and true feature, plus the MSE of the predicted (adversarial perturbed) feature and true features.  
\end{enumerate}

We tried sample based on certification result for unsafe1 states yet receive no improvement in terms of performance. We think it is mainly because as the vehicles gets close, the limit of the robustness boundary for those states becomes more narrow v.s. other states (where vehicles are far away). That apply adversarial training of all states and achieves global robust helps more w.r.t the certified result. Furthermore, focus on training unsafe1 states only also shows to result in lower nominal rewards, as the vehicles it interferes with the global stability of Q values and result in less optimal actions when the vehicles are close (unsafe 1).

\begin{table*}[]
\caption{For 2 NN only}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
                                     & avg cert & std cert & 75-perc time & 90-perc time & avg time & std time & timeout (10min) \\ \hline
5 steps                              & 4.5      & 0.8      & 0.11    & 0.28    & 0.09     & 0.12     & 0               \\ \hline
10 steps                             & 4.2      & 0.6      & 0.35    & 0.62    & 0.44     & 1.00        & 0               \\ \hline
15 steps                             & 3.7      & 1.2      & 4.96    & 10.00   & 3.16     & 3.95     & 3               \\ \hline
15 steps (cap eps based on 10 steps) & 3.7      & 1.2      & 1.26    & 3.91    & 1.47     & 2.73     & 1               \\ \hline
\end{tabular}
\end{table*}

\subsection{Notations}
MSE of feature: MSE between predicted feature on the nominal path v.s. the true feature on the nomianl path.

False action rate: the percentage of different actions where we take RL action based on predicted feature v.s. based on true feature.
